(4,2)-choosability of planar graphs with forbidden structures

All planar graphs are 4-colorable and 5-choosable, while some planar graphs are not 4-choosable. Determining which properties guarantee that a planar graph can be colored using lists of size four has received significant attention. In terms of constraining the structure of the graph, for any $\ell \in \{3,4,5,6,7\}$, a planar graph is 4-choosable if it is $\ell$-cycle-free. In terms of constraining the list assignment, one refinement of $k$-choosability is choosability with separation. A graph is $(k,s)$-choosable if the graph is colorable from lists of size $k$ where adjacent vertices have at most $s$ common colors in their lists. Every planar graph is $(4,1)$-choosable, but there exist planar graphs that are not $(4,3)$-choosable. It is an open question whether planar graphs are always $(4,2)$-choosable. A chorded $\ell$-cycle is an $\ell$-cycle with one additional edge. We demonstrate for each $\ell \in \{5,6,7\}$ that a planar graph is $(4,2)$-choosable if it does not contain chorded $\ell$-cycles.

==> figures/3pathsB-newpos.tex <==
\begin{tikzpicture}[vtx/.style={shape=coordinate}]


==> figures/advancedconfigs.tex <==
\begin{figure}[htp]
\centering

\begin{tabular}[h]{I}
\scalebox{0.8}{\input{figures/d9bg.tex}}
\\
\configuration{d9bg}
\end{tabular}
\
\begin{tabular}[h]{A}
\scalebox{0.8}{\input{figures/d9cf.tex}}
\\
\configuration{d9cf}
\end{tabular}
\
\begin{tabular}[h]{A}
\scalebox{0.8}{\input{figures/d9bgcf.tex}}
\\
\configuration{d9bgcf}
\end{tabular}
\ 
\begin{tabular}[h]{A}
\scalebox{0.8}{\input{figures/d8bf.tex}}
\\
\configuration{d8bf}
\end{tabular}

\begin{tabular}[h]{I}
\scalebox{0.8}{\input{figures/d4hk.tex}}
\\
\configuration{d4hk}
\end{tabular}
\ 
\begin{tabular}[h]{I}
\scalebox{0.8}{\input{figures/d4Bfk-smaller.tex}}
\\
\configuration{d4Bfk}
\end{tabular}
\ 
\begin{tabular}[h]{I}
\scalebox{0.8}{\input{figures/d4Bgk-smaller.tex}}
\\
\configuration{d4Bgk}
\end{tabular}
\ 
\begin{tabular}[h]{I}
\scalebox{0.8}{\input{figures/d4Bbg.tex}}
\\
\configuration{d4Bbg}
\end{tabular}


%
%\begin{tabular}[h]{I}
%\input{figures/d1be.tex}
%\\
%\configuration{d1be}
%\end{tabular}
%\ 
%
%&
%\input{figures/d7bg.tex}
%&
%\input{figures/d7cf.tex}
%&
%\configuration{d7bg} 
%&
%\configuration{d7cf} 
%\\[1ex]
%\input{figures/d7bgcf.tex}
%&
%\input{figures/d9bg.tex}
%&
%\input{figures/d9cf.tex}
%\\
%\configuration{d7bgcf}
%&
%\configuration{d9bg} 
%&
%\configuration{d9cf}  
%\\[1ex]
%\input{figures/d9bgcf.tex}
%&
%\input{figures/d8bf.tex}
%&
%\input{figures/d4hk.tex}
%\\
%\configuration{d9bgcf} 
%&
%\configuration{d8bf} 
%&
%\configuration{d4hk} 
%\\[1ex]
%\end{tabular}

\caption{\label{fig:advancedconfigs} More reducible configurations.}
\end{figure}

==> figures/bigconfiglist.tex <==


\scalebox{2.0}{
\input{figures/c1.tex}
\ref{cycle4}}


\scalebox{2.0}{
\input{figures/c2.tex}
\ref{cycle6}
}


\scalebox{2.0}{
\input{figures/c3.tex} 
 \ref{diamond1}
}


\scalebox{2.0}{
\input{figures/c4.tex}  
 \ref{diamond2}
}






\scalebox{2.0}{
\input{figures/c5.tex} 
\ref{4fan}
}



\scalebox{2.0}{
\input{figures/c6.tex}  
\ref{triforce}
}


\scalebox{2.0}{
\input{figures/c7.tex} 
\ref{4wheelplus}
}


\scalebox{2.0}{
\input{figures/c8.tex}
\ref{K6hconfig1}
}




\scalebox{2.0}{
\input{figures/c9.tex}  
}




\scalebox{2.0}{
\input{figures/c10.tex}
}




\scalebox{2.0}{
\input{figures/d11.tex} 
}




\scalebox{2.0}{
\input{figures/d2.tex}  
}


\scalebox{2.0}{
\input{figures/d1.tex}
}



\scalebox{2.0}{
\input{figures/d9.tex} 
}



\scalebox{2.0}{
\input{figures/d7.tex}
}




\scalebox{2.0}{
\input{figures/d5.tex} 
}




\scalebox{2.0}{
\input{figures/d6.tex} 
}




\scalebox{2.0}{
\input{figures/d8.tex} 
}





\scalebox{2.0}{
\input{figures/d4.tex}
}






\scalebox{2.0}{
\input{figures/d4b.tex}
}






\scalebox{2.0}{
\input{figures/d10.tex}
}


\scalebox{2.0}{
\input{figures/d1be.tex}
}





\scalebox{2.0}{
\input{figures/d7bg.tex}
}




\scalebox{2.0}{
\input{figures/d7cf.tex}
}




\scalebox{2.0}{
\input{figures/d7bgcf.tex}
}



\scalebox{2.0}{
\input{figures/d9bg.tex}
}


\scalebox{2.0}{
\input{figures/d9cf.tex}
}



\scalebox{2.0}{
\input{figures/d9bgcf.tex}
}



\scalebox{2.0}{
\input{figures/d8bf.tex}
}





\scalebox{2.0}{
\input{figures/d4hk.tex}
}



\scalebox{2.0}{
{\input{figures/d4Bfk-smaller.tex}}
}



\scalebox{2.0}{
{\input{figures/d4Bgk-smaller.tex}}
}



\scalebox{2.0}{
{\input{figures/d4Bbg.tex}}
}



